Developer Reactions to Protestware in Open Source Software: The cases of color.js and es5.ext

There is growing concern about maintainers self-sabotaging their work in order to take political or economic stances, a practice referred to as "protestware". Our objective is to understand the discourse around discussions on such an attack, how it is received by the community, and whether developers respond to the attack in a timely manner. We study two notable protestware cases i.e., colors.js and es5-ext. Results indicate that protestware discussions are spread more quickly on the GitHub platform, while security vulnerabilities are faster on social media. By establishing a taxonomy of protestware discussions, we identify posts that express stances and provide technical mitigation instructions. We applied a thematic analysis to 684 protestware related posts to identify five major themes during the discussions: i. disseminate and response, ii. stance, iii. reputation, iv. communicative styles, v. rights and ethics. This work sheds light on the nuanced landscape of protestware discussions, offering insights for both researchers and developers into maintaining a healthy balance between the political or social actions of developers and the collective well-being of the open-source community.

==> comments.tex <==
\usepackage[colorinlistoftodos]{todonotes}
\def\mybar#1{%%
  #1s & {\color{grey}\rule{#1cm}{8pt}}}


% \newcommand{\nb}[2]{
% 	{
% 		{\color{red}{
% 				\fbox{\bfseries\sffamily\scriptsize#1}
% 				{\sffamily$\triangleright~${\it\sffamily #2}$~\triangleleft$}
% 	}}}
% }


\definecolor{chestnut}{rgb}{0.8, 0.36, 0.36}


\newcommand\respond[2]{{\nb{#2}{\color{balck}#1}}}

% \newcommand{\impacttext}[1]{{\color{red}#1}}
\newcommand{\rone}[1]{\colorbox{blue}{\textbf{[#1]}}
\newcommand\revise[1]{\nb{Revised}{\color{balck}#1}}
\newcommand\youmei[1]{\nb{Freya}{\color{awesome}#1}}
\newcommand\asia[1]{\nb{Asia}{\color{red}#1}}
\newcommand\wang[1]{\nb{Wang}{\color{purple}#1}}
\newcommand\raula[1]{\nb{Raula}{\color{blue}#1}}
\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME] #1}}\xspace}
\newcommand{\cn}{{\color{violet}[citation required]}}
\newcommand{\tbd}{{\color{green}[To Be Done!]}}
\definecolor{chestnut}{rgb}{0.8, 0.36, 0.36}
